Efficient Parallel Solution of the 3D Stationary Boltzmann Transport Equation for Diffusive Problems

This paper presents an efficient parallel method for the deterministic solution of the 3D stationary Boltzmann transport equation applied to diffusive problems such as nuclear core criticality computations. Based on standard MultiGroup-Sn-DD discretization schemes, our approach combines a highly efficient nested parallelization strategy with the Piecewise Diffusion Synthetic Acceleration (PDSA) parallel technique applied for the first time to 3D transport problems. These two key ingredients enable us to solve extremely large neutronic problems involving up to $10^{12}$ degrees of freedom in less than an hour using 64 super-computer nodes.

==> figures/svg/cell_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/cell_2D.pdf}


==> figures/svg/flux_current_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/flux_current_RT0.pdf}


==> figures/svg/kobayashi_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1>[width=\linewidth]{\varFigRep/figures/svg/kobayashi_Problem1.pdf}
\includegraphics<2->[width=\linewidth]{\varFigRep/figures/svg/kobayashi_Problem2.pdf}


==> figures/svg/pdsa-comm_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/pdsa-comm_2SD.pdf}


==> figures/svg/pdsa_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1>[width=\linewidth]{\varFigRep/figures/svg/pdsa_Dirichlet.pdf}
\includegraphics<2>[width=\linewidth]{\varFigRep/figures/svg/pdsa_Neumann.pdf}
\includegraphics<3->[width=\linewidth]{\varFigRep/figures/svg/pdsa_Comm.pdf}


==> figures/svg/quadrants_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/quadrants_All.pdf}


==> figures/svg/rt0_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/rt0_2D.pdf}


==> figures/svg/sweep-2D-4X4-dag_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/sweep-2D-4X4-dag_Full.pdf}


==> figures/svg/sweep-2D-6X6-dag_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/sweep-2D-6X6-dag_Step2.pdf}


==> figures/svg/sweep-2D-6X6-grid_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/sweep-2D-6X6-grid_Step2.pdf}


==> figures/svg/takedaXY_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/takedaXY_Calque_1.pdf}


==> figures/svg/takedaXZ_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1->[width=\linewidth]{\varFigRep/figures/svg/takedaXZ_Calque_1.pdf}


==> figures/svg/takeda_include_slide.tex <==
\def\varFigRep{/home/plagne/gitProjects/DominoJCP/figures/svg/}
\includegraphics<1>[width=\linewidth]{\varFigRep/figures/svg/takeda_XY.pdf}
\includegraphics<2->[width=\linewidth]{\varFigRep/figures/svg/takeda_XZ.pdf}


==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

% \todo[inline]{List other acceleration schemes}

% \cite{denovo}, \cite{pentran2011}



==> source_iteration_accel.tex <==
\section{Acceleration of Source Iterations}
\label{sec:accel}



\todo[inline]{Explain the issue with the average value at corners, when
  using a multidimensional partitioning}
